TRIGO: Benchmarking Formal Mathematical Proof Reduction for Generative Language Models

Automated theorem proving (ATP) has become an appealing domain for exploring the reasoning ability of the recent successful generative language models. However, current ATP benchmarks mainly focus on symbolic inference, but rarely involve the understanding of complex number combination reasoning. In this work, we propose TRIGO, an ATP benchmark that not only requires a model to reduce a trigonometric expression with step-by-step proofs but also evaluates a generative LM's reasoning ability on formulas and its capability to manipulate, group, and factor number terms. We gather trigonometric expressions and their reduced forms from the web, annotate the simplification process manually, and translate it into the Lean formal language system. We then automatically generate additional examples from the annotated samples to expand the dataset. Furthermore, we develop an automatic generator based on Lean-Gym to create dataset splits of varying difficulties and distributions in order to thoroughly analyze the model's generalization ability. Our extensive experiments show our proposed TRIGO poses a new challenge for advanced generative LM's including GPT-4 which is pre-trained on a considerable amount of open-source formal theorem-proving language data, and provide a new tool to study the generative LM's ability on both formal and mathematical reasoning.

==> emnlp2023-latex/tab/GPT4-TAB.tex <==
\begin{table}[t]
\lstset{
    basicstyle=\tt,
    keywordstyle=\color{purple}\bfseries,
    identifierstyle=\color{black},
    commentstyle=\color{gray}
    showstringspaces=false,
    captionpos=b,                   	% 将标题位置设置为底部
    flexiblecolumns=true,
    breaklines=true,                	% 设置自动断行
    breakatwhitespace=false,        	% 设置自动中
    numbers=none,
}
\begin{tiny}
\begin{lstlisting}      
import data.real.basic
import analysis.special_functions.trigonometric.basic
open real
open_locale real
lemma Trigo_0 : sin(107 * π) = 0 :=
begin
  --Use the periodicity of the sine function:
  --sin(x+2*π*n) = sin(x) 
  for any integer n
  have h  : sin(107 * π) = sin(107 * π + 2 * π * -53),
  { rw sin_periodic_int_mul_pi (-53) },
  --Simplify the right-hand side of h 
  have h  : 107 * π + 2 * π * -53 = 54 * π,
  { rw [mul_comm 107, mul_comm 54], norm_num },
  --Combine h  and h , then use the sine of multiples of π
  rw [h , h , sin_mul_pi_of_ne_one 54],
end
\end{lstlisting}
We continue with the prompt: "We require to use lemma from Lean's standard library for the proof and to ensure the correctness of the equation."
\begin{lstlisting}      
import analysis.special_functions.trigonometric -- for sin, pi
open real
lemma sin_periodic : ∀ x : ℝ, sin x = sin (x + 2 * pi) :=
begin
  intros,
  exact sin_periodic_pi x, --available in Lean standard library
end

--Now we can prove the main result
lemma Trigo_0 : sin (107 * pi) = 0 :=
begin
  --Use the periodicity of sin to relate sin(107*pi) to sin(pi)
  have h : sin (107 * pi) = sin (1 * pi), 
  {
    apply sin_periodic,
  },
  --We know sin(pi) = 0
  rw h,
  exact sin_pi, --available in Lean standard library
end

\end{lstlisting}
\end{tiny}
\vspace{-4mm}
\caption{An example of GPT-4 struggling to solve a problem from \dataset.}
\label{tab:gpt4_example}
\vspace{-4mm}
\end{table}

==> emnlp2023-latex/tab/GPT4_have.tex <==
\begin{table}[t]
\lstset{
    basicstyle=\tt,
    keywordstyle=\color{purple}\bfseries,
    identifierstyle=\color{black},
    commentstyle=\color{gray}
    showstringspaces=false,
    captionpos=b,                   	% 将标题位置设置为底部
    flexiblecolumns=true,
    breaklines=true,                	% 设置自动断行
    breakatwhitespace=true,        	% 设置自动中
    numbers=none,
}
   
\begin{tiny}
\begin{lstlisting}      
GOAL ⊢ cos(433*pi/3) = 2*cos(pi/6)**2 - 1 
PROOFSTEP have : cos(pi/3) = cos(433*pi/3),
GPT-4 answer have : cos(2*pi/3) = 2*cos(pi/6)**2 - 1,

GOAL ⊢ cos(433*pi/3) = 2*cos(pi/6)**2 - 1 
PROOFSTEP have : cos(pi/3) = cos(433*pi/3),
GPT-4 answer have : cos(pi/3) = 2*cos(pi/6)**2 - 1,

GOAL h0 : tan(295*pi/6)≠0, this : tan(-pi/3) = (-1)/tan(295*pi/6) ⊢ sin(-pi/3)/cos(-pi/3) = tan(-pi/3) 
PROOFSTEP have : sin(-pi/3)/cos(-pi/3) = tan(-pi/3),
GPT-4 answer have : sin(-pi/3)/cos(-pi/3) = tan(-pi/3),

GOAL ⊢ sin(4*pi/3)*cos(pi/3) - sin(pi/3)*cos(4*pi/3) = 2*sin(pi/2)*cos(pi/2) 
PROOFSTEP have : sin(pi) = sin(4*pi/3)*cos(pi/3) - sin(pi/3)*cos(4*pi/3),
GPT-4 answer have : sin(4pi/3)*cos(pi/3) - sin(pi/3)*cos(4pi/3) = 2*sin(pi/2)*cos(pi/2),
\end{lstlisting}

\end{tiny}
\vspace{-4mm}
\caption{One-step proofs generated by GPT-4 using 8-shot examples.}
\label{tab:gpt4_have}
\vspace{-4mm}
\end{table}

==> emnlp2023-latex/tab/data.tex <==
import trigo_import
open real
open_locale real
variables (x y : ℝ)



lemma Trigo_0_0_RLMT : 3/4 - 3*sin(pi/12)**2/2=3*sqrt(3)/8:=
begin
  have : sin(pi/12)**2  =  1/2 - cos(pi/6)/2,
  {
  have : cos (pi/6) = cos(2*(pi/12)),
  {
  apply congr_arg,
  ring,
  },
  rw this,S
  rw cos_two_mul'',
  ring,
  },
  rw this,
  rw cos_pi_div_six,
  field_simp,
  ring_exp,
end

lemma Trigo_0_1_NBLH (h0 : cos(5*pi/6) ≠ 0) : 2*tan(5*pi/6)/(1 - tan(5*pi/6)**2)=-sqrt(3):=
begin
  have : 2*tan(5*pi/6)/(1 - tan(5*pi/6)**2)  =  tan(5*pi/3),
  {
  have : tan (5*pi/3) = tan(2*(5*pi/6)),
  {
  apply congr_arg,
  ring,
  },
  rw this,
  rw tan_two_mul,
  repeat {assumption},
  },
  rw this,
  have : tan(5*pi/3)  =  -tan(pi/3),
  {
  rw tan_eq_neg_tan_neg_add_int_mul_pi (5*pi/3) (2),
  repeat {apply congr_arg _},
  simp,
  linarith,
  },
  rw this,
  rw tan_pi_div_three,
end

lemma Trigo_0_2_LVJK : sin(pi/3) + 2*cos(pi/12)**2 - cos(pi/2)=sqrt(3)+1:=
begin
  rw cos_pi_div_two,
  rw sin_pi_div_three,
  have : cos(pi/12)**2  =  cos(pi/6)/2 + 1/2,
  {
  have : cos (pi/6) = cos(2*(pi/12)),
  {
  apply congr_arg,
  ring,
  },
  rw this,
  rw cos_two_mul,
  ring,
  },
  rw this,
  rw cos_pi_div_six,
  norm_num,
  field_simp,
  ring_exp,
end

lemma Trigo_0_3_NRRR : sin(pi/3)**2 + cos(pi/6)*cos(pi/3)=(3+sqrt(3))/4:=
begin
  rw cos_pi_div_six,
  rw cos_pi_div_three,
  rw sin_pi_div_three,
  norm_num,
  field_simp,
  ring_exp,
end

lemma Trigo_0_4_MQBL : sin(pi/4)*cos(pi/4)=1/2:=
begin
  rw sin_pi_div_four,
  rw cos_pi_div_four,
  field_simp,
end

lemma Trigo_0_5_QTWV : tan(3*pi/4)=-1:=
begin
  have : tan(3*pi/4)  =  -tan(pi/4),
  {
  rw tan_eq_neg_tan_neg_add_int_mul_pi (3*pi/4) (1),
  repeat {apply congr_arg _},
  simp,
  linarith,
  },
  rw this,
  rw tan_pi_div_four,
end

lemma Trigo_0_6_HTUW : sin(-2*pi/3)=-sqrt(3)/2:=
begin
  have : sin(-2*pi/3)  =  -sin(pi/3),
  {
  rw sin_eq_neg_sin_add_int_mul_two_pi_add_pi (-2*pi/3) (0),
  repeat {apply congr_arg _},
  simp,
  linarith,
  },
  rw this,
  rw sin_pi_div_three,
  field_simp,
end

lemma Trigo_0_7_HOEW : sin(23*pi/6)=-1/2:=
begin
  have : sin(23*pi/6)  =  -sin(pi/6),
  {
  rw sin_eq_neg_sin_neg_add_int_mul_two_pi (23*pi/6) (2),
  repeat {apply congr_arg _},
  simp,
  linarith,
  },
  rw this,
  rw sin_pi_div_six,
  norm_num,
end

lemma Trigo_0_8_LNDY : sin(2*pi/3)=sqrt(3)/2:=
begin
  have : sin(2*pi/3)  =  sin(pi/3),
  {
  rw sin_eq_sin_neg_add_int_mul_two_pi_add_pi (2*pi/3) (0),
  repeat {apply congr_arg _},
  simp,
  linarith,
  },
  rw this,
  rw sin_pi_div_three,
end

lemma Trigo_0_9_PWSS : sin(pi/12)*cos(pi/12)=1/4:=
begin
  have : sin(pi/12)*cos(pi/12)  =  sin(pi/6)/2,
  {
  have : sin(pi/6) = 2*sin(pi/12)*cos(pi/12),
  {
  have : sin (pi/6) = sin(2*(pi/12)),
  {
  apply congr_arg,
  ring,
  },
  rw this,
  rw sin_two_mul,
  },
  linarith,
  },
  rw this,
  rw sin_pi_div_six,
  norm_num,
end

lemma Trigo_0_10_JCYT : -sin(x)**2*sin(y)**2 - sin(x)**2*cos(y)**2 + sin(x)**2 + sin(y)**2=sin(y)**2:=
begin
  have : -sin(x)**2*sin(y)**2 - sin(x)**2*cos(y)**2  =  -sin(x)**2*(sin(y)**2 + cos(y)**2),
  {
  field_simp [-sin_sq_add_cos_sq, -cos_sq_add_sin_sq],
  ring_exp,
  },
  rw this,
  rw sin_sq_add_cos_sq,
  norm_num,
end

lemma Trigo_0_11_UPWT : -sin(23*pi/180)*cos(53*pi/180) + sin(53*pi/180)*cos(23*pi/180)=1/2:=
begin
  have : -sin(23*pi/180)*cos(53*pi/180) + sin(53*pi/180)*cos(23*pi/180)  =  sin(pi/6),
  {
  have : sin(pi/6) = sin((53*pi/180) - (23*pi/180)),
  {
  apply congr_arg,
  ring,
  },
  rw this,
  rw sin_sub,
  ring,
  },
  rw this,
  rw sin_pi_div_six,
end

lemma Trigo_0_12_KMNE : sin(pi/12)*cos(pi/12)/2=1/8:=
begin
  have : sin(pi/12)*cos(pi/12)/2  =  sin(pi/6)/4,
  {
  have : sin(pi/6) = 2*sin(pi/12)*cos(pi/12),
  {
  have : sin (pi/6) = sin(2*(pi/12)),
  {
  apply congr_arg,
  ring,
  },
  rw this,
  rw sin_two_mul,
  },
  linarith,
  },
  rw this,
  rw sin_pi_div_six,
  norm_num,
end

lemma Trigo_0_13_AURP : 2*sin(pi/3)=sqrt(3):=
begin
  rw sin_pi_div_three,
  field_simp,
  ring_exp,
end

lemma Trigo_0_14_HQRK : sin(23*pi/180)*cos(37*pi/180) + sin(37*pi/180)*cos(23*pi/180)=sqrt(3)/2:=
begin
  have : sin(23*pi/180)*cos(37*pi/180) + sin(37*pi/180)*cos(23*pi/180)  =  sin(pi/3),
  {
  have : sin(pi/3) = sin((23*pi/180) + (37*pi/180)),
  {
  apply congr_arg,
  ring,
  },
  rw this,
  rw sin_add,
  ring,
  },
  rw this,
  rw sin_pi_div_three,
end

lemma Trigo_0_15_ETRV : sin(5*pi/4) + tan(11*pi/3)=-sqrt(2)/2-sqrt(3):=
begin
  have : tan(11*pi/3)  =  tan(-pi/3),
  {
  rw tan_eq_tan_add_int_mul_pi (11*pi/3) (-4),
  repeat {apply congr_arg _},
  simp,
  linarith,
  },
  rw this,
  have : sin(5*pi/4)  =  -sin(pi/4),
  {
  rw sin_eq_neg_sin_add_int_mul_two_pi_add_pi (5*pi/4) (-1),
  repeat {apply congr_arg _},
  simp,
  linarith,
  },
  rw this,
  have : tan(-pi/3)  =  -tan(pi/3),
  {
  rw tan_eq_neg_tan_neg_add_int_mul_pi (-pi/3) (0),
  repeat {apply congr_arg _},
  simp,
  linarith,
  },
  rw this,
  rw tan_pi_div_three,
  rw sin_pi_div_four,
  field_simp,
  ring_exp,
end

lemma Trigo_0_16_ZMIB : -sin(pi/12)*sin(7*pi/12) + sin(5*pi/12)*sin(11*pi/12)=0:=
begin
  have : sin(7*pi/12)  =  cos(pi/12),
  {
  rw sin_eq_cos_add_pi_div_two_add_int_mul_two_pi_add_pi (7*pi/12) (-1),
  repeat {apply congr_arg _},
  simp,
  linarith,
  },
  rw this,
  have : sin(5*pi/12)  =  cos(pi/12),
  {
  rw sin_eq_cos_neg_add_pi_div_two_add_int_mul_two_pi (5*pi/12) (0),
  repeat {apply congr_arg _},
  simp,
  linarith,
  },
  rw this,
  have : sin(11*pi/12)  =  sin(pi/12),
  {
  rw sin_eq_sin_neg_add_int_mul_two_pi_add_pi (11*pi/12) (0),
  repeat {apply congr_arg _},
  simp,
  linarith,
  },
  rw this,
  norm_num,
  ring_exp,
end

lemma Trigo_0_17_FTGL : sin(-19*pi/6)=1/2:=
begin
  have : sin(-19*pi/6)  =  sin(-7*pi/6),
  {
  rw sin_eq_sin_add_int_mul_two_pi (-19*pi/6) (1),
  repeat {apply congr_arg _},
  simp,
  linarith,
  },
  rw this,
  have : sin(-7*pi/6)  =  -sin(7*pi/6),
  {
  rw sin_eq_neg_sin_neg_add_int_mul_two_pi (-7*pi/6) (0),
  repeat {apply congr_arg _},
  simp,
  linarith,
  },
  rw this,
  have : sin(7*pi/6)  =  -sin(pi/6),
  {
  rw sin_eq_neg_sin_add_int_mul_two_pi_add_pi (7*pi/6) (-1),
  repeat {apply congr_arg _},
  simp,
  linarith,
  },
  rw this,
  rw sin_pi_div_six,
  norm_num,
end

==> emnlp2023-latex/tab/expand_data.tex <==
import trigo_import
open real
open_locale real
variables (x y : ℝ)



lemma Trigo_0_0_RLMT_extend : 3/4 - 3*(-sin(-5*pi/12)*sin(173*pi) + sin(pi/2)*cos(677*pi/12))**2/2=3*sqrt(3)/8:=
begin
have : 3 / 4 - 3 * (sin((-5) * pi / 12) * -sin(173 * pi) + sin(pi / 2) * cos(677 * pi / 12)) ** 2 / 2 = 3/4 - 3*(-sin(-5*pi/12)*sin(173*pi) + sin(pi/2)*cos(677*pi/12))**2/2,
{
field_simp at *,
},
conv {to_lhs, rw ← this,},
have : cos(pi/2) = -sin(173*pi),
{
rw cos_eq_neg_sin_neg_add_pi_div_two_add_int_mul_two_pi_add_pi (pi/2) (86),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : 3 / 4 - 3 * (sin((-5) * pi / 12) * cos(pi / 2) + sin(pi / 2) * cos(677 * pi / 12)) ** 2 / 2 = 3/4 - 3*(sin(-5*pi/12)*cos(pi/2) + sin(pi/2)*cos(677*pi/12))**2/2,
{
field_simp at *,
},
have : cos(-5*pi/12) = cos(677*pi/12),
{
rw cos_eq_cos_neg_add_int_mul_two_pi (-5*pi/12) (28),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : 3 / 4 - 3 * (sin((-5) * pi / 12) * cos(pi / 2) + sin(pi / 2) * cos((-5) * pi / 12)) ** 2 / 2 = 3/4 - 3*(sin(-5*pi/12)*cos(pi/2) + sin(pi/2)*cos(-5*pi/12))**2/2,
{
field_simp at *,
},
have : sin(pi/12) = sin(-5*pi/12) * cos(pi/2) + sin(pi/2) * cos(-5*pi/12),
{
have : sin(pi/12) = sin((-5*pi/12) + (pi/2)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_add,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(pi/12)**2 = 1/2 - cos(pi/6)/2,
{
have : cos(pi/6) = cos(2*(pi/12)),
{
apply congr_arg,
ring,
},
rw this,
rw cos_two_mul'',
ring,
},
rw this,
rw cos_pi_div_six,
field_simp,
ring_exp,
end


lemma Trigo_0_1_NBLH_extend(h0 : cos(5*pi/6) ≠ 0)  (h1 : tan(209*pi/3)≠ 0) (h2 : (1-(1/tan(209*pi/3))**2)≠ 0) (h3 : ((1-1/tan(209*pi/3)**2)*tan(209*pi/3))≠ 0) (h4 : sin(209*pi/3)≠ 0) (h5 : cos(209*pi/3)≠ 0) (h6 : (sin(209*pi/3)/cos(209*pi/3))≠ 0) (h7 : ((-cos(209*pi/3)**2/sin(209*pi/3)**2+1)*sin(209*pi/3))≠ 0) (h8 : ((1-1/(sin(209*pi/3)/cos(209*pi/3))**2)*(sin(209*pi/3)/cos(209*pi/3)))≠ 0) (h9 : ((-cos(467*pi/3)**2/sin(209*pi/3)**2+1)*sin(209*pi/3))≠ 0) : 2*cos(467*pi/3)/((-cos(467*pi/3)**2/sin(209*pi/3)**2 + 1)*sin(209*pi/3))=-sqrt(3):=
begin
have : cos(209*pi/3) = cos(467*pi/3),
{
rw cos_eq_cos_add_int_mul_two_pi (209*pi/3) (43),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : 2 / ((1 - 1 / (sin(209 * pi / 3) / cos(209 * pi / 3)) ** 2) * (sin(209 * pi / 3) / cos(209 * pi / 3))) = 2*cos(209*pi/3)/((-cos(209*pi/3)**2/sin(209*pi/3)**2 + 1)*sin(209*pi/3)),
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : tan(209*pi/3) = sin(209*pi/3) / cos(209*pi/3),
{
rw tan_eq_sin_div_cos,
},
conv {to_lhs, rw ← this,},
have : 2 * (1 / tan(209 * pi / 3)) / (1 - (1 / tan(209 * pi / 3)) ** 2) = 2/((1 - 1/tan(209*pi/3)**2)*tan(209*pi/3)),
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : tan(5*pi/6) = 1 / tan(209*pi/3),
{
rw tan_eq_one_div_tan_neg_add_pi_div_two_add_int_mul_pi (5*pi/6) (70),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : 2*tan(5*pi/6)/(1 - tan(5*pi/6)**2) = tan(5*pi/3),
{
have : tan(5*pi/3) = tan(2*(5*pi/6)),
{
apply congr_arg,
ring,
},
rw this,
rw tan_two_mul,
repeat {assumption},
},
rw this,
have : tan(5*pi/3) = -tan(pi/3),
{
rw tan_eq_neg_tan_neg_add_int_mul_pi (5*pi/3) (2),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
rw tan_pi_div_three,
end


lemma Trigo_0_2_LVJK_extend (h0 : cos(pi/3)≠ 0) (h1 : (2*cos(pi/3))≠ 0) (h2 : sin(pi/12)≠ 0) (h3 : (2*sin(pi/12))≠ 0) (h4 : (2*sin(pi/12)**2)≠ 0) : -cos(pi/2) + sin(62*pi/3)/(2*cos(pi/3)) + sin(pi/6)**2/(2*sin(pi/12)**2)=sqrt(3)+1:=
begin
have : -cos(pi / 2) + sin(62 * pi / 3) / (2 * cos(pi / 3)) + 2 * (sin(pi / 6) / (2 * sin(pi / 12))) ** 2 = -cos(pi/2) + sin(62*pi/3)/(2*cos(pi/3)) + sin(pi/6)**2/(2*sin(pi/12)**2),
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : cos(pi/12) = sin(pi/6) / ( 2 * sin(pi/12) ),
{
have : sin(pi/6) = sin(2*(pi/12)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_two_mul,
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(2*pi/3) = sin(62*pi/3),
{
rw sin_eq_sin_add_int_mul_two_pi (2*pi/3) (10),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(2 * pi / 3) / (2 * cos(pi / 3)) + 2 * cos(pi / 12) ** 2 - cos(pi / 2) = -cos(pi/2) + sin(2*pi/3)/(2*cos(pi/3)) + 2*cos(pi/12)**2,
{
field_simp at *,
},
conv {to_lhs, rw ← this,},
have : sin(pi/3) = sin(2*pi/3) / ( 2 * cos(pi/3) ),
{
have : sin(2*pi/3) = sin(2*(pi/3)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_two_mul,
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
rw cos_pi_div_two,
rw sin_pi_div_three,
have : cos(pi/12)**2 = cos(pi/6)/2 + 1/2,
{
have : cos(pi/6) = cos(2*(pi/12)),
{
apply congr_arg,
ring,
},
rw this,
rw cos_two_mul,
ring,
},
rw this,
rw cos_pi_div_six,
norm_num,
field_simp,
ring_exp,
end


lemma Trigo_0_3_NRRR_extend : -cos(437*pi/3)*cos(955*pi/6) + sin(pi/3)**2=(3+sqrt(3))/4:=
begin
have : cos(58*pi/3) = -cos(437*pi/3),
{
rw cos_eq_neg_cos_neg_add_int_mul_two_pi_add_pi (58*pi/3) (82),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : - -cos(58 * pi / 3) * cos(955 * pi / 6) + sin(pi / 3) ** 2 = cos(58*pi/3)*cos(955*pi/6) + sin(pi/3)**2,
{
field_simp at *,
},
conv {to_lhs, rw ← this,},
have : cos(pi/3) = -cos(58*pi/3),
{
rw cos_eq_neg_cos_add_int_mul_two_pi_add_pi (pi/3) (9),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(pi / 3) ** 2 + -cos(955 * pi / 6) * cos(pi / 3) = -cos(pi/3)*cos(955*pi/6) + sin(pi/3)**2,
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : cos(pi/6) = -cos(955*pi/6),
{
rw cos_eq_neg_cos_add_int_mul_two_pi_add_pi (pi/6) (79),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
rw cos_pi_div_six,
rw cos_pi_div_three,
rw sin_pi_div_three,
norm_num,
field_simp,
ring_exp,
end


lemma Trigo_0_4_MQBL_extend : -sin(0)/2 - sin(359*pi/2)/2=1/2:=
begin
have : sin(343*pi/2) = sin(359*pi/2),
{
rw sin_eq_sin_add_int_mul_two_pi (343*pi/2) (4),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : -sin(0) / 2 + -sin(343 * pi / 2) / 2 = -sin(0)/2 - sin(343*pi/2)/2,
{
field_simp at *,
},
conv {to_lhs, rw ← this,},
have : sin(pi/2) = -sin(343*pi/2),
{
rw sin_eq_neg_sin_add_int_mul_two_pi_add_pi (pi/2) (85),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(pi/4) * cos(pi/4) = -sin(0) / 2 + sin(pi/2) / 2,
{
rw mul_comm,
rw cos_mul_sin,
have : sin((pi/4) + (pi/4)) = sin(pi/2),
{
apply congr_arg,
ring,
},
rw this,
have : sin((pi/4) - (pi/4)) = sin(0),
{
apply congr_arg,
ring,
},
rw this,
ring,
},
conv {to_lhs, rw ← this,},
have : (sin(pi/4) * cos(pi/4)) = sin(pi/4)*cos(pi/4),
{
ring,
},
rw sin_pi_div_four,
rw cos_pi_div_four,
field_simp,
end


lemma Trigo_0_5_QTWV_extend (h0 : cos(3*pi/8)≠ 0) (h1 : (1-tan(3*pi/8)**2)≠ 0) (h2 : tan(689*pi/8)≠ 0) (h3 : ((1-1/tan(689*pi/8)**2)*tan(689*pi/8))≠ 0) (h4 : (1-(1/tan(689*pi/8))**2)≠ 0) (h5 : cos((689*pi/4)/2)≠ 0) (h6 : (sin(689*pi/4)/(1+cos(689*pi/4)))≠ 0) (h7 : ((-(cos(689*pi/4)+1)**2/sin(689*pi/4)**2+1)*sin(689*pi/4))≠ 0) (h8 : ((1-1/(sin(689*pi/4)/(1+cos(689*pi/4)))**2)*(sin(689*pi/4)/(1+cos(689*pi/4))))≠ 0) (h9 : sin(689*pi/4)≠ 0) (h10 : (1+cos(689*pi/4))≠ 0) : 2*(cos(689*pi/4) + 1)/((-(cos(689*pi/4) + 1)**2/sin(689*pi/4)**2 + 1)*sin(689*pi/4))=-1:=
begin
have : 2 / ((1 - 1 / (sin(689 * pi / 4) / (1 + cos(689 * pi / 4))) ** 2) * (sin(689 * pi / 4) / (1 + cos(689 * pi / 4)))) = 2*(cos(689*pi/4) + 1)/((-(cos(689*pi/4) + 1)**2/sin(689*pi/4)**2 + 1)*sin(689*pi/4)),
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : tan(689*pi/8) = sin(689*pi/4) / ( 1 + cos(689*pi/4) ),
{
have : tan(689*pi/8) = tan((689*pi/4)/2),
{
apply congr_arg,
ring,
},
rw this,
rw tan_div_two',
repeat {assumption},
},
conv {to_lhs, rw ← this,},
have : 2 * (1 / tan(689 * pi / 8)) / (1 - (1 / tan(689 * pi / 8)) ** 2) = 2/((1 - 1/tan(689*pi/8)**2)*tan(689*pi/8)),
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : tan(3*pi/8) = 1 / tan(689*pi/8),
{
rw tan_eq_one_div_tan_neg_add_pi_div_two_add_int_mul_pi (3*pi/8) (86),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : tan(3*pi/4) = 2 * tan(3*pi/8) / ( 1 - tan(3*pi/8) ** 2 ),
{
have : tan(3*pi/4) = tan(2*(3*pi/8)),
{
apply congr_arg,
ring,
},
rw this,
rw tan_two_mul,
repeat {assumption},
},
conv {to_lhs, rw ← this,},
have : tan(3*pi/4) = -tan(pi/4),
{
rw tan_eq_neg_tan_neg_add_int_mul_pi (3*pi/4) (1),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
rw tan_pi_div_four,
end


lemma Trigo_0_6_HTUW_extend : 3*sin(-367*pi/9) - 4*sin(-367*pi/9)**3=-sqrt(3)/2:=
begin
have : (-4) * sin((-367) * pi / 9) ** 3 + 3 * sin((-367) * pi / 9) = 3*sin(-367*pi/9) - 4*sin(-367*pi/9)**3,
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(-367*pi/3) = -4 * sin(-367*pi/9) ** 3 + 3 * sin(-367*pi/9),
{
have : sin(-367*pi/3) = sin(3*(-367*pi/9)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_three_mul,
ring,
},
conv {to_lhs, rw ← this,},
have : - -sin((-367) * pi / 3) = sin(-367*pi/3),
{
field_simp at *,
},
conv {to_lhs, rw ← this,},
have : sin(463*pi/3) = -sin(-367*pi/3),
{
rw sin_eq_neg_sin_neg_add_int_mul_two_pi (463*pi/3) (16),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(-2*pi/3) = -sin(463*pi/3),
{
rw sin_eq_neg_sin_add_int_mul_two_pi_add_pi (-2*pi/3) (77),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(-2*pi/3) = -sin(pi/3),
{
rw sin_eq_neg_sin_add_int_mul_two_pi_add_pi (-2*pi/3) (0),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
rw sin_pi_div_three,
field_simp,
end


lemma Trigo_0_7_HOEW_extend : -2*sin(709*pi/12)*cos(709*pi/12)=-1/2:=
begin
have : -(2 * sin(709 * pi / 12) * cos(709 * pi / 12)) = -2*sin(709*pi/12)*cos(709*pi/12),
{
field_simp at *,
},
conv {to_lhs, rw ← this,},
have : sin(709*pi/6) = 2 * sin(709*pi/12) * cos(709*pi/12),
{
have : sin(709*pi/6) = sin(2*(709*pi/12)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_two_mul,
},
conv {to_lhs, rw ← this,},
have : sin(163*pi/6) = -sin(709*pi/6),
{
rw sin_eq_neg_sin_add_int_mul_two_pi_add_pi (163*pi/6) (45),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(23*pi/6) = sin(163*pi/6),
{
rw sin_eq_sin_neg_add_int_mul_two_pi_add_pi (23*pi/6) (15),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(23*pi/6) = -sin(pi/6),
{
rw sin_eq_neg_sin_neg_add_int_mul_two_pi (23*pi/6) (2),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
rw sin_pi_div_six,
norm_num,
end


lemma Trigo_0_8_LNDY_extend : 4*(-sin(pi/2)*cos(43*pi/18) + sin(43*pi/18)*cos(pi/2))**3 - 3*sin(43*pi/18)*cos(pi/2) + 3*sin(pi/2)*cos(43*pi/18)=sqrt(3)/2:=
begin
have : 4 * (sin(43 * pi / 18) * cos(pi / 2) - sin(pi / 2) * cos(43 * pi / 18)) ** 3 - 3 * (sin(43 * pi / 18) * cos(pi / 2) - sin(pi / 2) * cos(43 * pi / 18)) = 4*(-sin(pi/2)*cos(43*pi/18) + sin(43*pi/18)*cos(pi/2))**3 - 3*sin(43*pi/18)*cos(pi/2) + 3*sin(pi/2)*cos(43*pi/18),
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(17*pi/9) = sin(43*pi/18) * cos(pi/2) - sin(pi/2) * cos(43*pi/18),
{
have : sin(17*pi/9) = sin((43*pi/18) - (pi/2)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_sub,
ring,
},
conv {to_lhs, rw ← this,},
have : -((-4) * sin(17 * pi / 9) ** 3 + 3 * sin(17 * pi / 9)) = 4*sin(17*pi/9)**3 - 3*sin(17*pi/9),
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(17*pi/3) = -4 * sin(17*pi/9) ** 3 + 3 * sin(17*pi/9),
{
have : sin(17*pi/3) = sin(3*(17*pi/9)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_three_mul,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(2*pi/3) = -sin(17*pi/3),
{
rw sin_eq_neg_sin_add_int_mul_two_pi_add_pi (2*pi/3) (2),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(2*pi/3) = sin(pi/3),
{
rw sin_eq_sin_neg_add_int_mul_two_pi_add_pi (2*pi/3) (0),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
rw sin_pi_div_three,
end


lemma Trigo_0_9_PWSS_extend : -sin(2189*pi/12)*cos(3905*pi/12)=1/4:=
begin
have : cos(pi/12) = sin(2189*pi/12),
{
rw cos_eq_sin_neg_add_pi_div_two_add_int_mul_two_pi (pi/12) (91),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : -cos(3905 * pi / 12) * cos(pi / 12) = -cos(pi/12)*cos(3905*pi/12),
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(2195*pi/12) = -cos(3905*pi/12),
{
rw sin_eq_neg_cos_add_pi_div_two_add_int_mul_two_pi (2195*pi/12) (71),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(pi/12) = sin(2195*pi/12),
{
rw sin_eq_sin_neg_add_int_mul_two_pi_add_pi (pi/12) (91),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(pi/12)*cos(pi/12) = sin(pi/6)/2,
{
have : sin(pi/6) = 2*sin(pi/12)*cos(pi/12),
{
have : sin(pi/6) = sin(2*(pi/12)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_two_mul,
},
linarith,
},
rw this,
rw sin_pi_div_six,
norm_num,
end


lemma Trigo_0_10_JCYT_extend : -(1 - cos(-y + 371*pi/2)**2)*cos(x + 355*pi/2)**2 - sin(y)**2*cos(x + 355*pi/2)**2 + sin(y)**2 + cos(x + 355*pi/2)**2=sin(y)**2:=
begin
have : -sin(y) ** 2 * cos(x + 355 * pi / 2) ** 2 + sin(y) ** 2 - (1 - cos(-y + 371 * pi / 2) ** 2) * cos(x + 355 * pi / 2) ** 2 + cos(x + 355 * pi / 2) ** 2 = -(1 - cos(-y + 371*pi/2)**2)*cos(x + 355*pi/2)**2 - sin(y)**2*cos(x + 355*pi/2)**2 + sin(y)**2 + cos(x + 355*pi/2)**2,
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(-y + 371*pi/2) ** 2 = 1 - cos(-y + 371*pi/2) ** 2,
{
rw sin_sq,
},
conv {to_lhs, rw ← this,},
have : -cos(x + 355 * pi / 2) ** 2 * sin(y) ** 2 - cos(x + 355 * pi / 2) ** 2 * sin(-y + 371 * pi / 2) ** 2 + cos(x + 355 * pi / 2) ** 2 + sin(y) ** 2 = -sin(y)**2*cos(x + 355*pi/2)**2 + sin(y)**2 - sin(-y + 371*pi/2)**2*cos(x + 355*pi/2)**2 + cos(x + 355*pi/2)**2,
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(x) = cos(x + 355*pi/2),
{
rw sin_eq_cos_add_pi_div_two_add_int_mul_two_pi_add_pi (x) (88),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : -sin(x) ** 2 * sin(y) ** 2 - sin(x) ** 2 * (-sin(-y + 371 * pi / 2)) ** 2 + sin(x) ** 2 + sin(y) ** 2 = -sin(x)**2*sin(y)**2 - sin(x)**2*sin(-y + 371*pi/2)**2 + sin(x)**2 + sin(y)**2,
{
field_simp at *,
},
conv {to_lhs, rw ← this,},
have : cos(y) = -sin(-y + 371*pi/2),
{
rw cos_eq_neg_sin_neg_add_pi_div_two_add_int_mul_two_pi_add_pi (y) (92),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : -sin(x)**2*sin(y)**2 - sin(x)**2*cos(y)**2 = -sin(x)**2*(sin(y)**2 + cos(y)**2),
{
field_simp [-sin_sq_add_cos_sq, -cos_sq_add_sin_sq],
ring_exp,
},
rw this,
rw sin_sq_add_cos_sq,
norm_num,
end


lemma Trigo_0_11_UPWT_extend : -sin(23*pi/180)*cos(-8693*pi/180) - sin(-pi/6)/2 + sin(19*pi/45)/2=1/2:=
begin
have : sin(23 * pi / 180) * -cos((-8693) * pi / 180) - sin(-pi / 6) / 2 + sin(19 * pi / 45) / 2 = -sin(23*pi/180)*cos(-8693*pi/180) - sin(-pi/6)/2 + sin(19*pi/45)/2,
{
field_simp at *,
},
conv {to_lhs, rw ← this,},
have : sin(29843*pi/180) = -cos(-8693*pi/180),
{
rw sin_eq_neg_cos_neg_add_pi_div_two_add_int_mul_two_pi_add_pi (29843*pi/180) (58),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : -sin(23 * pi / 180) * -sin(29843 * pi / 180) - sin(-pi / 6) / 2 + sin(19 * pi / 45) / 2 = sin(23*pi/180)*sin(29843*pi/180) - sin(-pi/6)/2 + sin(19*pi/45)/2,
{
field_simp at *,
},
conv {to_lhs, rw ← this,},
have : cos(53*pi/180) = -sin(29843*pi/180),
{
rw cos_eq_neg_sin_add_pi_div_two_add_int_mul_two_pi_add_pi (53*pi/180) (82),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : -sin(23 * pi / 180) * cos(53 * pi / 180) + (-sin(-pi / 6) / 2 + sin(19 * pi / 45) / 2) = -sin(23*pi/180)*cos(53*pi/180) - sin(-pi/6)/2 + sin(19*pi/45)/2,
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(53*pi/180) * cos(23*pi/180) = -sin(-pi/6) / 2 + sin(19*pi/45) / 2,
{
rw mul_comm,
rw cos_mul_sin,
have : sin((23*pi/180) + (53*pi/180)) = sin(19*pi/45),
{
apply congr_arg,
ring,
},
rw this,
have : sin((23*pi/180) - (53*pi/180)) = sin(-pi/6),
{
apply congr_arg,
ring,
},
rw this,
ring,
},
conv {to_lhs, rw ← this,},
have : (sin(53*pi/180) * cos(23*pi/180)) = sin(53*pi/180)*cos(23*pi/180),
{
ring,
},
have : -sin(23*pi/180)*cos(53*pi/180) + sin(53*pi/180)*cos(23*pi/180) = sin(pi/6),
{
have : sin(pi/6) = sin((53*pi/180) - (23*pi/180)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_sub,
ring,
},
rw this,
rw sin_pi_div_six,
end


lemma Trigo_0_12_KMNE_extend : -sin(1405*pi/12)*cos(239*pi/12)/2=1/8:=
begin
have : cos(pi/12) = cos(239*pi/12),
{
rw cos_eq_cos_neg_add_int_mul_two_pi (pi/12) (10),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(1213*pi/12) = sin(1405*pi/12),
{
rw sin_eq_sin_add_int_mul_two_pi (1213*pi/12) (8),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(pi/12) = -sin(1213*pi/12),
{
rw sin_eq_neg_sin_add_int_mul_two_pi_add_pi (pi/12) (50),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(pi/12)*cos(pi/12)/2 = sin(pi/6)/4,
{
have : sin(pi/6) = 2*sin(pi/12)*cos(pi/12),
{
have : sin(pi/6) = sin(2*(pi/12)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_two_mul,
},
linarith,
},
rw this,
rw sin_pi_div_six,
norm_num,
end


lemma Trigo_0_13_AURP_extend : -4*sin(pi/12)*sin(1061*pi/12)*cos(pi/2) + 2*sin(pi/2)*cos(pi/6)=sqrt(3):=
begin
have : (-4) * sin(pi / 12) * sin(1061 * pi / 12) * cos(pi / 2) + 2 * sin(pi / 2) * cos(pi / 6) = -4*sin(pi/12)*sin(1061*pi/12)*cos(pi/2) + 2*sin(pi/2)*cos(pi/6),
{
field_simp at *,
},
have : cos(pi/12) = sin(1061*pi/12),
{
rw cos_eq_sin_neg_add_pi_div_two_add_int_mul_two_pi (pi/12) (44),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : (-2) * (2 * sin(pi / 12) * cos(pi / 12)) * cos(pi / 2) + 2 * sin(pi / 2) * cos(pi / 6) = -4*sin(pi/12)*cos(pi/12)*cos(pi/2) + 2*sin(pi/2)*cos(pi/6),
{
field_simp at *,
},
conv {to_lhs, rw ← this,},
have : sin(pi/6) = 2 * sin(pi/12) * cos(pi/12),
{
have : sin(pi/6) = sin(2*(pi/12)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_two_mul,
},
conv {to_lhs, rw ← this,},
have : 2 * (sin(pi / 2) * cos(pi / 6) - sin(pi / 6) * cos(pi / 2)) = -2*sin(pi/6)*cos(pi/2) + 2*sin(pi/2)*cos(pi/6),
{
field_simp at *,
},
conv {to_lhs, rw ← this,},
have : sin(pi/3) = sin(pi/2) * cos(pi/6) - sin(pi/6) * cos(pi/2),
{
have : sin(pi/3) = sin((pi/2) - (pi/6)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_sub,
ring,
},
conv {to_lhs, rw ← this,},
rw sin_pi_div_three,
field_simp,
ring_exp,
end


lemma Trigo_0_14_HQRK_extend (h0 : sin(19403*pi/180)≠ 0) (h1 : (2*sin(19403*pi/180))≠ 0) (h2 : sin(19403*pi/180)≠ 0) : sin(23*pi/360)*sin(19403*pi/90)*cos(23*pi/360)/sin(19403*pi/180) + sin(37*pi/180)*cos(23*pi/180)=sqrt(3)/2:=
begin
have : 2 * sin(23 * pi / 360) * cos(23 * pi / 360) * sin(19403 * pi / 90) / (2 * sin(19403 * pi / 180)) + sin(37 * pi / 180) * cos(23 * pi / 180) = sin(23*pi/360)*sin(19403*pi/90)*cos(23*pi/360)/sin(19403*pi/180) + sin(37*pi/180)*cos(23*pi/180),
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(23*pi/180) = 2 * sin(23*pi/360) * cos(23*pi/360),
{
have : sin(23*pi/180) = sin(2*(23*pi/360)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_two_mul,
},
conv {to_lhs, rw ← this,},
have : sin(23 * pi / 180) * (sin(19403 * pi / 90) / (2 * sin(19403 * pi / 180))) + sin(37 * pi / 180) * cos(23 * pi / 180) = sin(23*pi/180)*sin(19403*pi/90)/(2*sin(19403*pi/180)) + sin(37*pi/180)*cos(23*pi/180),
{
field_simp at *,
},
conv {to_lhs, rw ← this,},
have : cos(19403*pi/180) = sin(19403*pi/90) / ( 2 * sin(19403*pi/180) ),
{
have : sin(19403*pi/90) = sin(2*(19403*pi/180)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_two_mul,
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : cos(37*pi/180) = cos(19403*pi/180),
{
rw cos_eq_cos_neg_add_int_mul_two_pi (37*pi/180) (54),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(23*pi/180)*cos(37*pi/180) + sin(37*pi/180)*cos(23*pi/180) = sin(pi/3),
{
have : sin(pi/3) = sin((23*pi/180) + (37*pi/180)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_add,
ring,
},
rw this,
rw sin_pi_div_three,
end


lemma Trigo_0_15_ETRV_extend : tan(11*pi/3) + (sin(-pi)*sin(pi) + cos(-pi)*cos(pi))*sin(-3*pi/4) + sin(-2*pi)*sin(225*pi/4)=-sqrt(2)/2-sqrt(3):=
begin
have : tan(11 * pi / 3) + sin((-3) * pi / 4) * (sin(-pi) * sin(pi) + cos(-pi) * cos(pi)) + sin((-2) * pi) * sin(225 * pi / 4) = tan(11*pi/3) + (sin(-pi)*sin(pi) + cos(-pi)*cos(pi))*sin(-3*pi/4) + sin(-2*pi)*sin(225*pi/4),
{
field_simp at *,
},
conv {to_lhs, rw ← this,},
have : cos(-2*pi) = sin(-pi) * sin(pi) + cos(-pi) * cos(pi),
{
have : cos(-2*pi) = cos((-pi) - (pi)),
{
apply congr_arg,
ring,
},
rw this,
rw cos_sub,
ring,
},
conv {to_lhs, rw ← this,},
have : tan(11 * pi / 3) + sin((-3) * pi / 4) * cos((-2) * pi) - sin((-2) * pi) * -sin(225 * pi / 4) = tan(11*pi/3) + sin(-3*pi/4)*cos(-2*pi) + sin(-2*pi)*sin(225*pi/4),
{
field_simp at *,
},
conv {to_lhs, rw ← this,},
have : cos(-3*pi/4) = -sin(225*pi/4),
{
rw cos_eq_neg_sin_neg_add_pi_div_two_add_int_mul_two_pi_add_pi (-3*pi/4) (27),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin((-3) * pi / 4) * cos((-2) * pi) - sin((-2) * pi) * cos((-3) * pi / 4) + tan(11 * pi / 3) = tan(11*pi/3) + sin(-3*pi/4)*cos(-2*pi) - sin(-2*pi)*cos(-3*pi/4),
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(5*pi/4) = sin(-3*pi/4) * cos(-2*pi) - sin(-2*pi) * cos(-3*pi/4),
{
have : sin(5*pi/4) = sin((-3*pi/4) - (-2*pi)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_sub,
ring,
},
conv {to_lhs, rw ← this,},
have : tan(11*pi/3) = tan(-pi/3),
{
rw tan_eq_tan_add_int_mul_pi (11*pi/3) (-4),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
have : sin(5*pi/4) = -sin(pi/4),
{
rw sin_eq_neg_sin_add_int_mul_two_pi_add_pi (5*pi/4) (-1),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
have : tan(-pi/3) = -tan(pi/3),
{
rw tan_eq_neg_tan_neg_add_int_mul_pi (-pi/3) (0),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
rw tan_pi_div_three,
rw sin_pi_div_four,
field_simp,
ring_exp,
end


lemma Trigo_0_16_ZMIB_extend (h0 : cos(pi/12)≠ 0) (h1 : (2*cos(pi/12))≠ 0) : (sin(229*pi/4)/2 - sin(673*pi/12)/2)/(2*cos(pi/12)) + sin(5*pi/12)*sin(11*pi/12)=0:=
begin
have : (-sin(673 * pi / 12) / 2 + sin(229 * pi / 4) / 2) / (2 * cos(pi / 12)) + sin(5 * pi / 12) * sin(11 * pi / 12) = (sin(229*pi/4)/2 - sin(673*pi/12)/2)/(2*cos(pi/12)) + sin(5*pi/12)*sin(11*pi/12),
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(7*pi/12) * cos(170*pi/3) = -sin(673*pi/12) / 2 + sin(229*pi/4) / 2,
{
rw mul_comm,
rw cos_mul_sin,
have : sin((170*pi/3) + (7*pi/12)) = sin(229*pi/4),
{
apply congr_arg,
ring,
},
rw this,
have : sin((170*pi/3) - (7*pi/12)) = sin(673*pi/12),
{
apply congr_arg,
ring,
},
rw this,
ring,
},
conv {to_lhs, rw ← this,},
have : (sin(7*pi/12) * cos(170*pi/3))/(2*cos(pi/12)) = sin(7*pi/12)*cos(170*pi/3)/(2*cos(pi/12)),
{
ring,
},
have : - -cos(170 * pi / 3) * sin(7 * pi / 12) / (2 * cos(pi / 12)) + sin(5 * pi / 12) * sin(11 * pi / 12) = sin(7*pi/12)*cos(170*pi/3)/(2*cos(pi/12)) + sin(5*pi/12)*sin(11*pi/12),
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(pi/6) = -cos(170*pi/3),
{
rw sin_eq_neg_cos_add_pi_div_two_add_int_mul_two_pi (pi/6) (28),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : -(sin(pi / 6) / (2 * cos(pi / 12))) * sin(7 * pi / 12) + sin(5 * pi / 12) * sin(11 * pi / 12) = -sin(pi/6)*sin(7*pi/12)/(2*cos(pi/12)) + sin(5*pi/12)*sin(11*pi/12),
{
field_simp at *,
},
conv {to_lhs, rw ← this,},
have : sin(pi/12) = sin(pi/6) / ( 2 * cos(pi/12) ),
{
have : sin(pi/6) = sin(2*(pi/12)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_two_mul,
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(7*pi/12) = cos(pi/12),
{
rw sin_eq_cos_add_pi_div_two_add_int_mul_two_pi_add_pi (7*pi/12) (-1),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
have : sin(5*pi/12) = cos(pi/12),
{
rw sin_eq_cos_neg_add_pi_div_two_add_int_mul_two_pi (5*pi/12) (0),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
have : sin(11*pi/12) = sin(pi/12),
{
rw sin_eq_sin_neg_add_int_mul_two_pi_add_pi (11*pi/12) (0),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
norm_num,
ring_exp,
end


lemma Trigo_0_17_FTGL_extend : -sin(967*pi/6)=1/2:=
begin
have : cos(-113*pi/3) = -sin(967*pi/6),
{
rw cos_eq_neg_sin_neg_add_pi_div_two_add_int_mul_two_pi_add_pi (-113*pi/3) (61),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : - -cos((-113) * pi / 3) = cos(-113*pi/3),
{
field_simp at *,
},
conv {to_lhs, rw ← this,},
have : sin(1003*pi/6) = -cos(-113*pi/3),
{
rw sin_eq_neg_cos_neg_add_pi_div_two_add_int_mul_two_pi_add_pi (1003*pi/6) (64),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(-19*pi/6) = -sin(1003*pi/6),
{
rw sin_eq_neg_sin_neg_add_int_mul_two_pi (-19*pi/6) (82),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(-19*pi/6) = sin(-7*pi/6),
{
rw sin_eq_sin_add_int_mul_two_pi (-19*pi/6) (1),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
have : sin(-7*pi/6) = -sin(7*pi/6),
{
rw sin_eq_neg_sin_neg_add_int_mul_two_pi (-7*pi/6) (0),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
have : sin(7*pi/6) = -sin(pi/6),
{
rw sin_eq_neg_sin_add_int_mul_two_pi_add_pi (7*pi/6) (-1),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
rw sin_pi_div_six,
norm_num,
end


lemma Trigo_0_18_TPOC_extend : -2*sin(221*pi/12)*cos(691*pi/12)=-1/2:=
begin
have : 2 * sin(221 * pi / 12) * -cos(691 * pi / 12) = -2*sin(221*pi/12)*cos(691*pi/12),
{
field_simp at *,
},
conv {to_lhs, rw ← this,},
have : cos(7*pi/12) = -cos(691*pi/12),
{
rw cos_eq_neg_cos_add_int_mul_two_pi_add_pi (7*pi/12) (28),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(7*pi/12) = sin(221*pi/12),
{
rw sin_eq_sin_neg_add_int_mul_two_pi_add_pi (7*pi/12) (9),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(7*pi/6) = 2 * sin(7*pi/12) * cos(7*pi/12),
{
have : sin(7*pi/6) = sin(2*(7*pi/12)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_two_mul,
},
conv {to_lhs, rw ← this,},
have : sin(7*pi/6) = -sin(pi/6),
{
rw sin_eq_neg_sin_add_int_mul_two_pi_add_pi (7*pi/6) (-1),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
rw sin_pi_div_six,
norm_num,
end


lemma Trigo_0_19_TYCU_extend (h0 : cos(11*pi/60)≠ 0) (h1 : (2*cos(11*pi/60))≠ 0) (h2 : (2*cos(4331*pi/60))≠ 0) : sin(3*pi/20)*cos(4331*pi/60) + (-sin(3*pi/40)**2 + cos(3*pi/40)**2)*sin(11*pi/30)/(2*cos(4331*pi/60))=sqrt(3)/2:=
begin
have : cos(11*pi/60) = cos(4331*pi/60),
{
rw cos_eq_cos_add_int_mul_two_pi (11*pi/60) (36),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(3 * pi / 20) * cos(11 * pi / 60) + sin(11 * pi / 30) * (-sin(3 * pi / 40) ** 2 + cos(3 * pi / 40) ** 2) / (2 * cos(11 * pi / 60)) = sin(3*pi/20)*cos(11*pi/60) + (-sin(3*pi/40)**2 + cos(3*pi/40)**2)*sin(11*pi/30)/(2*cos(11*pi/60)),
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : cos(3*pi/20) = -sin(3*pi/40) ** 2 + cos(3*pi/40) ** 2,
{
have : cos(3*pi/20) = cos(2*(3*pi/40)),
{
apply congr_arg,
ring,
},
rw this,
rw cos_two_mul',
ring,
},
conv {to_lhs, rw ← this,},
have : sin(3 * pi / 20) * cos(11 * pi / 60) + sin(11 * pi / 30) / (2 * cos(11 * pi / 60)) * cos(3 * pi / 20) = sin(3*pi/20)*cos(11*pi/60) + sin(11*pi/30)*cos(3*pi/20)/(2*cos(11*pi/60)),
{
field_simp at *,
},
conv {to_lhs, rw ← this,},
have : sin(11*pi/60) = sin(11*pi/30) / ( 2 * cos(11*pi/60) ),
{
have : sin(11*pi/30) = sin(2*(11*pi/60)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_two_mul,
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(3*pi/20)*cos(11*pi/60) + sin(11*pi/60)*cos(3*pi/20) = sin(pi/3),
{
have : sin(pi/3) = sin((3*pi/20) + (11*pi/60)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_add,
ring,
},
rw this,
rw sin_pi_div_three,
end


lemma Trigo_0_20_BOHO_extend : (sin(pi/4)*sin(190*pi/3) + sin(pi/6)*cos(pi/4))*sin(5*pi/6) + sin(190*pi/3)*cos(1885*pi/12)=sqrt(2)/2:=
begin
have : -(-sin(pi / 6) * cos(pi / 4) + sin(pi / 4) * -sin(190 * pi / 3)) * sin(5 * pi / 6) - -sin(190 * pi / 3) * cos(1885 * pi / 12) = (sin(pi/4)*sin(190*pi/3) + sin(pi/6)*cos(pi/4))*sin(5*pi/6) + sin(190*pi/3)*cos(1885*pi/12),
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : cos(pi/6) = -sin(190*pi/3),
{
rw cos_eq_neg_sin_neg_add_pi_div_two_add_int_mul_two_pi_add_pi (pi/6) (31),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : -(sin(pi / 4) * cos(pi / 6) - sin(pi / 6) * cos(pi / 4)) * sin(5 * pi / 6) - cos(pi / 6) * cos(1885 * pi / 12) = -(-sin(pi/6)*cos(pi/4) + sin(pi/4)*cos(pi/6))*sin(5*pi/6) - cos(pi/6)*cos(1885*pi/12),
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(pi/12) = sin(pi/4) * cos(pi/6) - sin(pi/6) * cos(pi/4),
{
have : sin(pi/12) = sin((pi/4) - (pi/6)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_sub,
ring,
},
conv {to_lhs, rw ← this,},
have : -sin(pi / 12) * sin(5 * pi / 6) + -cos(1885 * pi / 12) * cos(pi / 6) = -sin(pi/12)*sin(5*pi/6) - cos(pi/6)*cos(1885*pi/12),
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(5*pi/12) = -cos(1885*pi/12),
{
rw sin_eq_neg_cos_neg_add_pi_div_two_add_int_mul_two_pi_add_pi (5*pi/12) (78),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(5*pi/12) = cos(pi/12),
{
rw sin_eq_cos_neg_add_pi_div_two_add_int_mul_two_pi (5*pi/12) (0),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
have : sin(5*pi/6) = sin(pi/6),
{
rw sin_eq_sin_neg_add_int_mul_two_pi_add_pi (5*pi/6) (0),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
have : -sin(pi/12)*sin(pi/6) + cos(pi/12)*cos(pi/6) = cos(pi/4),
{
have : cos(pi/4) = cos((pi/6) + (pi/12)),
{
apply congr_arg,
ring,
},
rw this,
rw cos_add,
ring,
},
rw this,
rw cos_pi_div_four,
end


lemma Trigo_0_21_DDDQ_extend (h0 : sin(9*pi/4)≠ 0) (h1 : (2*sin(9*pi/4))≠ 0) : -tan(191*pi/6) + sin(193*pi/2)/(2*sin(9*pi/4))=(3*sqrt(2)+2*sqrt(3))/6:=
begin
have : sin(9*pi/2) = sin(193*pi/2),
{
rw sin_eq_sin_neg_add_int_mul_two_pi_add_pi (9*pi/2) (50),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : cos(9*pi/4) = sin(9*pi/2) / ( 2 * sin(9*pi/4) ),
{
have : sin(9*pi/2) = sin(2*(9*pi/4)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_two_mul,
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : cos(9 * pi / 4) + -tan(191 * pi / 6) = -tan(191*pi/6) + cos(9*pi/4),
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : tan(-11*pi/6) = -tan(191*pi/6),
{
rw tan_eq_neg_tan_neg_add_int_mul_pi (-11*pi/6) (30),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : tan(-11*pi/6) = tan(pi/6),
{
rw tan_eq_tan_add_int_mul_pi (-11*pi/6) (2),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
rw tan_pi_div_six,
have : cos(9*pi/4) = cos(pi/4),
{
rw cos_eq_cos_add_int_mul_two_pi (9*pi/4) (-1),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
rw cos_pi_div_four,
field_simp,
ring_exp,
end


lemma Trigo_0_22_WAJU_extend (h0 : (cos(-pi/3)+2*cos(4*pi/3)**2+2)≠ 0) (h1 : (2*cos(4*pi/3)**2+cos(-pi/3)+2)≠ 0) (h2 : sin(4*pi/3)≠ 0) (h3 : (2*sin(4*pi/3))≠ 0) (h4 : (2*(sin(8*pi/3)/(2*sin(4*pi/3)))**2+cos(-pi/3)+2)≠ 0) (h5 : (sin(8*pi/3)**2/(2*sin(4*pi/3)**2)+cos(-pi/3)+2)≠ 0) (h6 : (2*sin(4*pi/3)**2)≠ 0) (h7 : (-3*cos(-pi/9)+sin(8*pi/3)**2/(2*sin(4*pi/3)**2)+2+4*cos(-pi/9)**3)≠ 0) (h8 : (sin(8*pi/3)**2/(2*sin(4*pi/3)**2)+(4*cos(-pi/9)**3-3*cos(-pi/9))+2)≠ 0) : (-3 - 2*sin(1135*pi/6)**3 + sin(5*pi/6) + sin(5*pi/3)**2)/(-3*cos(-pi/9) + sin(8*pi/3)**2/(2*sin(4*pi/3)**2) + 2 + 4*cos(-pi/9)**3)=-1/2:=
begin
have : (-3 - 2 * sin(1135 * pi / 6) ** 3 + sin(5 * pi / 6) + sin(5 * pi / 3) ** 2) / (sin(8 * pi / 3) ** 2 / (2 * sin(4 * pi / 3) ** 2) + (4 * cos(-pi / 9) ** 3 - 3 * cos(-pi / 9)) + 2) = (-3 - 2*sin(1135*pi/6)**3 + sin(5*pi/6) + sin(5*pi/3)**2)/(-3*cos(-pi/9) + sin(8*pi/3)**2/(2*sin(4*pi/3)**2) + 2 + 4*cos(-pi/9)**3),
{
field_simp at *,
repeat {left},
ring,
},
conv {to_lhs, rw ← this,},
have : cos(-pi/3) = 4 * cos(-pi/9) ** 3 - 3 * cos(-pi/9),
{
have : cos(-pi/3) = cos(3*(-pi/9)),
{
apply congr_arg,
ring,
},
rw this,
rw cos_three_mul,
},
conv {to_lhs, rw ← this,},
have : (-3 - 2 * sin(1135 * pi / 6) ** 3 + sin(5 * pi / 6) + sin(5 * pi / 3) ** 2) / (2 * (sin(8 * pi / 3) / (2 * sin(4 * pi / 3))) ** 2 + cos(-pi / 3) + 2) = (-3 - 2*sin(1135*pi/6)**3 + sin(5*pi/6) + sin(5*pi/3)**2)/(sin(8*pi/3)**2/(2*sin(4*pi/3)**2) + cos(-pi/3) + 2),
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : cos(4*pi/3) = sin(8*pi/3) / ( 2 * sin(4*pi/3) ),
{
have : sin(8*pi/3) = sin(2*(4*pi/3)),
{
apply congr_arg,
ring,
},
rw this,
rw sin_two_mul,
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : (sin(5 * pi / 6) + sin(5 * pi / 3) ** 2 + 2 * (-sin(1135 * pi / 6)) ** 3 - 3) / (cos(-pi / 3) + 2 * cos(4 * pi / 3) ** 2 + 2) = (-3 - 2*sin(1135*pi/6)**3 + sin(5*pi/6) + sin(5*pi/3)**2)/(2*cos(4*pi/3)**2 + cos(-pi/3) + 2),
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : cos(pi/3) = -sin(1135*pi/6),
{
rw cos_eq_neg_sin_neg_add_pi_div_two_add_int_mul_two_pi_add_pi (pi/3) (94),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
rw cos_pi_div_three,
have : sin(5*pi/6) = sin(pi/6),
{
rw sin_eq_sin_neg_add_int_mul_two_pi_add_pi (5*pi/6) (0),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
rw sin_pi_div_six,
have : sin(5*pi/3) = -sin(pi/3),
{
rw sin_eq_neg_sin_neg_add_int_mul_two_pi (5*pi/3) (1),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
rw sin_pi_div_three,
have : cos(-pi/3) = cos(pi/3),
{
rw cos_eq_cos_neg_add_int_mul_two_pi (-pi/3) (0),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
rw cos_pi_div_three,
have : cos(4*pi/3) = -cos(pi/3),
{
rw cos_eq_neg_cos_add_int_mul_two_pi_add_pi (4*pi/3) (-1),
repeat {apply congr_arg _},
simp,
linarith,
},
rw this,
rw cos_pi_div_three,
norm_num,
end


lemma Trigo_0_23_YNNF_extend : -sqrt(3)/2 - sin(1181*pi/4)*cos(473*pi/4) + sqrt(3)*cos(473*pi/4)**2=1/2:=
begin
have : -sqrt 3 / 2 + -sin(1181 * pi / 4) * cos(473 * pi / 4) + sqrt 3 * cos(473 * pi / 4) ** 2 = -sqrt(3)/2 - sin(1181*pi/4)*cos(473*pi/4) + sqrt(3)*cos(473*pi/4)**2,
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(497*pi/4) = -sin(1181*pi/4),
{
rw sin_eq_neg_sin_add_int_mul_two_pi_add_pi (497*pi/4) (85),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : -sqrt 3 / 2 + sin(497 * pi / 4) * cos(473 * pi / 4) + sqrt 3 * cos(473 * pi / 4) ** 2 = -sqrt(3)/2 + sin(497*pi/4)*cos(473*pi/4) + sqrt(3)*cos(473*pi/4)**2,
{
field_simp at *,
},
have : sin(pi/4) = sin(497*pi/4),
{
rw sin_eq_sin_add_int_mul_two_pi (pi/4) (62),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
have : sin(pi / 4) * cos(473 * pi / 4) + sqrt 3 * cos(473 * pi / 4) ** 2 - sqrt 3 / 2 = -sqrt(3)/2 + sin(pi/4)*cos(473*pi/4) + sqrt(3)*cos(473*pi/4)**2,
{
field_simp at *,
ring,
},
conv {to_lhs, rw ← this,},
have : cos(pi/4) = cos(473*pi/4),
{
rw cos_eq_cos_add_int_mul_two_pi (pi/4) (59),
focus{repeat {apply congr_arg _}},
simp,
ring,
},
conv {to_lhs, rw ← this,},
rw sin_pi_div_four,
rw cos_pi_div_four,
norm_num,
field_simp,
ring_exp,
end


==> emnlp2023-latex/tab/expert_iteration_result.tex <==

\begin{table}[!htb]
    \centering
    
    \scalebox{1.0}{
    \begin{tabular}{lcccc}
    \toprule
    Iteration & \multicolumn{3}{c}{\dataset-gen} \\
    & TG-1 & TG-2  & TG-3  \\
    \midrule
    0 & 77.29 & 44.19 & 18.99 \\
    1 & 81.39 & 54.59 & 19.99 \\
    2 & 80.79 & 55.39 & 24.39\\
    3 & 80.19 & 55.09 & 22.89\\
    4 & 80.69 & 57.29 & 23.69\\
    5 & 79.59 & 58.19 & 22.49\\
    6 & 81.69 & 55.99 & 24.09\\
    7 & 83.19 & 55.09 & 24.99\\
    \bottomrule
    \end{tabular}
    }
    \vspace{-4mm}
    \caption{\yuanye{Change to line chart.}Pass rate of different expert iteration steps.}
    \label{tab:expert_iteration_result}
    \vspace{-4mm}
\end{table}

==> emnlp2023-latex/tab/main_result.tex <==
\begin{table}[!htb]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
    \multirow{2}{*}{Model} & \multirow{2}{*}{\# Parameters}  & \multicolumn{3}{c}{Pass-rate (\%)} \\
    & & \dataset-real & \dataset-web & Merge\\
    \midrule
    \textit{Baseline} \\
    refl & - & 0.00 & 0.00 & 0.00 \\
    tidy & -  & 3.49 & 6.84 & 6.31\\
    \midrule
    \textit{Raw training} \\
    GPT2-B  & 117M & 13.95 & 15.01 & 14.84\\
    GPT2-L/28 & 607M & 23.26 & 17.22 & 18.18 \\
    GPT2-L & 762M & 19.77 & 15.23 & 15.95\\
    \midrule
    \textit{Parsed training} \\
    GPT2-B  & 117M & 17.44 & 16.78 & 16.88\\
    GPT2-L/28 & 607M & 24.42 & 18.32& 19.29 \\
    GPT2-L & 762M & 27.91  &18.10 & 19.67\\
    \midrule
    \textit{PACT + Raw training} \\
    GPT2-L/28 & 607M & 19.77 & 15.23 & 15.95\\
    \midrule
    \textit{PACT + Parsed training} \\
    GPT2-L/28 & 607M & \textbf{30.23} & \textbf{18.54} & \textbf{20.41}\\
    \bottomrule
    \end{tabular}
    }
    \vspace{-4mm}
    \caption{Pass rates of benchmark models and baselines.}
    \label{tab:main_result}
    \vspace{-4mm}
\end{table}

==> emnlp2023-latex/tab/rule_bank.tex <==
\begin{table*}[!htb]
    \centering
    %\setlength\extrarowheight{1.5 pt}
    \begin{tabular}{ccc}
    \toprule
    Identity Rule Name & Example \\
    \midrule
    Reflections & $sin(-X) = -sin(X)$\\
    Shifts and Periodicity & $sin(X + \pi/2) = cos(X)$ \\
    Pythagorean & $sin^2(X) + cos^2(X) = 1$  \\
    Angle sum and difference & $sin(X+Y) = sin(X)cos(Y) + cos(X)sin(Y)$ \\
    Product-to-sum & $sin(X)cos(Y) = (sin(X+Y)+sin(X-Y))/2$ \\
    Sum-to-product & $sin(X) + sin(Y) = 2sin((X+Y)/2)cos((X-Y)/2)$ \\
    Double-angle & $sin(2X) = 2sin(X)cos(X)$ \\
    Power-reduction & $sin^2(X) = (1-cos(2X))/2$\\
    Trigonometry value of special angles     & $sin(\pi/2) = 1$  \\
    Tangent definition & $cos(X) \ne 0 \rightarrow tan(X) = sin(X)/cos(X)$ \\
    Basic calculation & $(A+B)*C = A*C + B*C$ \\
    Absolute value & $X \ge 0 \rightarrow |X| = X$\\
    \bottomrule
    \end{tabular}
    \vspace{-4mm}
    \caption{Examples of identities in our pre-defined rule bank.}
    \label{tab:rules}
    \vspace{-4mm}
\end{table*}

==> emnlp2023-latex/tab/subgoal.tex <==
\begin{table}[htb]
\centering
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{lccc}
\toprule
Model& Single & Hierarchy & Both \\
\midrule
GPT2-L/28+Raw & 68.75 & 21.90   & 55.49\\
GPT2-L/28+Parsed & 77.08  & 41.90 & 66.38\\
\bottomrule
\end{tabular}}
\vspace{-4mm}
\caption{Pass rates of subgoals. ``Single'' denotes subgoals that do not contain another \textit{have} tactic in their proofs, and ``Hierarchy'' denotes the opposite.}
\label{tab:subgoal}
\vspace{-4mm}
\end{table}



==> lstlean.tex <==
% Listing style definition for the Lean Theorem Prover.
% Defined by Jeremy Avigad, 2015, by modifying Assia Mahboubi's SSR style.
% Unicode replacements taken from Olivier Verdier's unixode.sty

\lstdefinelanguage{lean} {

% Anything betweeen $ becomes LaTeX math mode
mathescape=false,
% Comments may or not include Latex commands
texcl=false,

% keywords, list taken from lean-syntax.el
morekeywords=[1]{
open_locale,import, prelude, protected, private, noncomputable, definition, meta, renaming,
hiding, exposing, parameter, parameters, begin, conjecture, constant, constants,
hypothesis, lemma, corollary, variable, variables, premise, premises, theory,
print, theorem, proposition, example,
open, as, export, override, axiom, axioms, inductive, with, without,
structure, record, universe, universes,
alias, help, precedence, reserve, declare_trace, add_key_equivalence,
match, infix, infixl, infixr, notation, postfix, prefix, instance,
eval, vm_eval, check, coercion, end, this, suppose,
using, using_well_founded, namespace, section, fields,
attribute, local, set_option, extends, include, omit, classes, class,
instances, coercions, attributes, raw, replacing,
calc, have, show, suffices, by, in, at, let, forall, Pi, fun,
exists, if, dif, then, else, assume, obtain, from, aliases, register_simp_ext, unless, break, continue,
mutual, do, def, run_cmd, const
partial,mut,where,macro,syntax,deriving, return, try, catch, for, macro_rules,declare_syntax_cat,abbrev},

% Sorts
morekeywords=[2]{Sort, Type, Prop},

% tactics, list taken from lean-syntax.el
morekeywords=[3]{
assumption,
apply, intro, intros, allGoals,
generalize, clear, revert, done, exact,
refine, repeat, cases, rewrite, rw,
simp, simp_all, contradiction, linarith, ring, conv, field_simp, 
constructor, injection,
induction,
contrapose,
obviously,
norm_num
},

% modifiers, taken from lean-syntax.el
% note: 'otherkeywords' is needed because these use a different symbol.
% this command doesn't allow us to specify a number -- they are put with [1]
% otherkeywords={
% [persistent], [notation], [visible], [instance], [trans_instance],
% [class], [parsing-only], [coercion], [unfold_full], [constructor],
% [reducible], [irreducible], [semireducible], [quasireducible], [wf],
% [whnf], [multiple_instances], [none], [decl], [declaration],
% [relation], [symm], [subst], [refl], [trans], [simp], [congr], [unify],
% [backward], [forward], [no_pattern], [begin_end], [tactic], [abbreviation],
% [reducible], [unfold], [alias], [eqv], [intro], [intro!], [elim], [grinder],
% [localrefinfo], [recursor]
% },

% Various symbols
literate=
{α}{{\ensuremath{\mathrm{\alpha}}}}1
{β}{{\ensuremath{\mathrm{\beta}}}}1
{γ}{{\ensuremath{\mathrm{\gamma}}}}1
{δ}{{\ensuremath{\mathrm{\delta}}}}1
{ε}{{\ensuremath{\mathrm{\varepsilon}}}}1
{ζ}{{\ensuremath{\mathrm{\zeta}}}}1
{η}{{\ensuremath{\mathrm{\eta}}}}1
{θ}{{\ensuremath{\mathrm{\theta}}}}1
{ι}{{\ensuremath{\mathrm{\iota}}}}1
{κ}{{\ensuremath{\mathrm{\kappa}}}}1
{μ}{{\ensuremath{\mathrm{\mu}}}}1
{ν}{{\ensuremath{\mathrm{\nu}}}}1
{ξ}{{\ensuremath{\mathrm{\xi}}}}1
{π}{{\ensuremath{\mathrm{\mathnormal{\pi}}}}}1
{ρ}{{\ensuremath{\mathrm{\rho}}}}1
{σ}{{\ensuremath{\mathrm{\sigma}}}}1
{τ}{{\ensuremath{\mathrm{\tau}}}}1
{φ}{{\ensuremath{\mathrm{\varphi}}}}1
{χ}{{\ensuremath{\mathrm{\chi}}}}1
{ψ}{{\ensuremath{\mathrm{\psi}}}}1
{ω}{{\ensuremath{\mathrm{\omega}}}}1

{Γ}{{\ensuremath{\mathrm{\Gamma}}}}1
{Δ}{{\ensuremath{\mathrm{\Delta}}}}1
{Θ}{{\ensuremath{\mathrm{\Theta}}}}1
{Λ}{{\ensuremath{\mathrm{\Lambda}}}}1
{Σ}{{\ensuremath{\mathrm{\Sigma}}}}1
{Φ}{{\ensuremath{\mathrm{\Phi}}}}1
{Ξ}{{\ensuremath{\mathrm{\Xi}}}}1
{Ψ}{{\ensuremath{\mathrm{\Psi}}}}1
{Ω}{{\ensuremath{\mathrm{\Omega}}}}1

{ℵ}{{\ensuremath{\aleph}}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1
{≠}{{\ensuremath{\neq}}}1
{≈}{{\ensuremath{\approx}}}1
{≡}{{\ensuremath{\equiv}}}1
{≃}{{\ensuremath{\simeq}}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1

{∂}{{\ensuremath{\partial}}}1
{∆}{{\ensuremath{\triangle}}}1 % or \laplace?

{∫}{{\ensuremath{\int}}}1
{∑}{{\ensuremath{\mathrm{\Sigma}}}}1
{Π}{{\ensuremath{\mathrm{\Pi}}}}1

{⊥}{{\ensuremath{\perp}}}1
{∞}{{\ensuremath{\infty}}}1
{∂}{{\ensuremath{\partial}}}1

{∓}{{\ensuremath{\mp}}}1
{±}{{\ensuremath{\pm}}}1
{×}{{\ensuremath{\times}}}1

{⊕}{{\ensuremath{\oplus}}}1
{⊗}{{\ensuremath{\otimes}}}1
{⊞}{{\ensuremath{\boxplus}}}1

{∇}{{\ensuremath{\nabla}}}1
{√}{{\ensuremath{\sqrt}}}1

{⬝}{{\ensuremath{\cdot}}}1
{•}{{\ensuremath{\cdot}}}1
{∘}{{\ensuremath{\circ}}}1

%{⁻}{{\ensuremath{^{\textup{\kern1pt\rule{2pt}{0.3pt}\kern-1pt}}}}}1
{⁻}{{\ensuremath{^{-}}}}1
{▸}{{\ensuremath{\blacktriangleright}}}1

{∧}{{\ensuremath{\wedge}}}1
{∨}{{\ensuremath{\vee}}}1
{¬}{{\ensuremath{\neg}}}1
{⊢}{{\ensuremath{\vdash}}}1

%{⟨}{{\ensuremath{\left\langle}}}1
%{⟩}{{\ensuremath{\right\rangle}}}1
{⟨}{{\ensuremath{\langle}}}1
{⟩}{{\ensuremath{\rangle}}}1

{↦}{{\ensuremath{\mapsto}}}1
{←}{{\ensuremath{\leftarrow}}}1
{<-}{{\ensuremath{\leftarrow}}}1
{→}{{\ensuremath{\rightarrow}}}1
{↔}{{\ensuremath{\leftrightarrow}}}1
{⇒}{{\ensuremath{\Rightarrow}}}1
{⟹}{{\ensuremath{\Longrightarrow}}}1
{⇐}{{\ensuremath{\Leftarrow}}}1
{⟸}{{\ensuremath{\Longleftarrow}}}1

{∩}{{\ensuremath{\cap}}}1
{∪}{{\ensuremath{\cup}}}1
{⊂}{{\ensuremath{\subseteq}}}1
{⊆}{{\ensuremath{\subseteq}}}1
{⊄}{{\ensuremath{\nsubseteq}}}1
{⊈}{{\ensuremath{\nsubseteq}}}1
{⊃}{{\ensuremath{\supseteq}}}1
{⊇}{{\ensuremath{\supseteq}}}1
{⊅}{{\ensuremath{\nsupseteq}}}1
{⊉}{{\ensuremath{\nsupseteq}}}1
{∈}{{\ensuremath{\in}}}1
{∉}{{\ensuremath{\notin}}}1
{∋}{{\ensuremath{\ni}}}1
{∌}{{\ensuremath{\notni}}}1
{∅}{{\ensuremath{\emptyset}}}1

{∖}{{\ensuremath{\setminus}}}1
{†}{{\ensuremath{\dag}}}1

{ℕ}{{\ensuremath{\mathbb{N}}}}1
{ℤ}{{\ensuremath{\mathbb{Z}}}}1
{ℝ}{{\ensuremath{\mathbb{R}}}}1
{ℚ}{{\ensuremath{\mathbb{Q}}}}1
{ℂ}{{\ensuremath{\mathbb{C}}}}1
{⌞}{{\ensuremath{\llcorner}}}1
{⌟}{{\ensuremath{\lrcorner}}}1
{⦃}{{\ensuremath{\{\!|}}}1
{⦄}{{\ensuremath{|\!\}}}}1

{‖}{{\ensuremath{\|}}}1
{₁}{{\ensuremath{_1}}}1
{₂}{{\ensuremath{_2}}}1
{₃}{{\ensuremath{_3}}}1
{₄}{{\ensuremath{_4}}}1
{₅}{{\ensuremath{_5}}}1
{₆}{{\ensuremath{_6}}}1
{₇}{{\ensuremath{_7}}}1
{₈}{{\ensuremath{_8}}}1
{₉}{{\ensuremath{_9}}}1
{₀}{{\ensuremath{_0}}}1
{ᵢ}{{\ensuremath{_i}}}1
{ⱼ}{{\ensuremath{_j}}}1
{ₐ}{{\ensuremath{_a}}}1

{¹}{{\ensuremath{^1}}}1

{ₙ}{{\ensuremath{_n}}}1
{ₘ}{{\ensuremath{_m}}}1
{↑}{{\ensuremath{\uparrow}}}1
{↓}{{\ensuremath{\downarrow}}}1

{...}{{\ensuremath{\ldots}}}1
{·}{{\ensuremath{\cdot}}}1

{▸}{{\ensuremath{\triangleright}}}1

{Σ}{{\color{symbolcolor}\ensuremath{\Sigma}}}1
{Π}{{\color{symbolcolor}\ensuremath{\Pi}}}1
{∀}{{\color{symbolcolor}\ensuremath{\forall}}}1
{∃}{{\color{symbolcolor}\ensuremath{\exists}}}1
{λ}{{\color{symbolcolor}\ensuremath{\mathrm{\lambda}}}}1
{\$}{{\color{symbolcolor}\$}}1

{:=}{{\color{symbolcolor}:=}}1
{=}{{\color{symbolcolor}=}}1
{<|>}{{\color{symbolcolor}<|>}}1
{<\$>}{{\color{symbolcolor}<\$>}}1
{+}{{\color{symbolcolor}+}}1
{*}{{\color{symbolcolor}*}}1,

% Comments
%comment=[s][\itshape \color{commentcolor}]{/-}{-/},
morecomment=[s][\color{commentcolor}]{/-}{-/},
morecomment=[l][\itshape \color{commentcolor}]{--},

% Spaces are not displayed as a special character
showstringspaces=false,

% keep spaces
keepspaces=true,

% String delimiters
morestring=[b]",
morestring=[d],

% Size of tabulations
tabsize=3,

% Enables ASCII chars 128 to 255
extendedchars=false,

% Case sensitivity
sensitive=true,

% Automatic breaking of long lines
breaklines=true,
breakatwhitespace=true,

% Default style fors listingsred
basicstyle=\ttfamily\small,

% Position of captions is bottom
captionpos=b,

% Full flexible columns
columns=[l]fullflexible,


% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the begining of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\color{keywordcolor}},

% Style for sorts
keywordstyle=[2]{\ttfamily\color{sortcolor}},

% Style for tactics keywords
keywordstyle=[3]{\ttfamily\color{tacticcolor}},

% Style for attributes
keywordstyle=[4]{\ttfamily\color{attributecolor}},

% Style for strings
stringstyle=\ttfamily,

% Style for comments
commentstyle={\ttfamily\footnotesize },

}
